Ion and neutral molecules in the W43-MM1(G30.79 FIR 10) infalling clump

The high mass star forming clump W43-MM1 has been mapped in N$_{2}$H$^{+}(4 \rightarrow 3)$, C$^{18}$O$(3 \rightarrow 2)$, SiO$(8 \rightarrow 7)$, and in a single pointing in DCO$^{+}(5 \rightarrow 4)$ towards the center of the clump. Column densities from these observations as well as previous HCO$^{+}(4 \rightarrow 3)$, H$^{13}$CO$^{+}(4 \rightarrow 3)$, HCN$(4 \rightarrow 3)$, H$^{13}$CN$(4 \rightarrow 3)$, and CS$(7 \rightarrow 6)$ data, have been derived using the RADEX code, results later used to derived chemical abundances at selected points in the MM1 main axis. Comparing with chemical models, we estimate an evolutionary age of $10^{4}$ years for a remarkable warm hot core inside MM1. We also proposed that the dust temperature derived from SED fitting in MM1 is not representative of the gas temperature deep inside the clump as dust emission may have become optically thick. By deriving a deuterium fractionation of $1.2 \times 10^{3}$, we estimate an electron fraction of $X(e)= 6.5 \times 10^{-8}$. Thus, the coupling between the neutral gas and the magnetic field is estimated by computing the ambipolar diffusion Reynolds number $R_{m}=18$ and the wave coupling number W=110. Considering that the infalling speed is slightly supersonic (M=1.1) but sub-alfvenic, we conclude that the MM1 clump has recently or is in the process of decoupling the field from the neutral fluid. Thus, the MM1 clump appears to be in an intermediate stage of evolution in which a hot core has developed while the envelope is still infalling and not fully decoupled from the ambient magnetic field.

==> tab3_old.tex <==
\begin{table*}
\centering                           % used for centering table
\caption[]{Hydrogen column densities derived from 1.3 mm data from \citet{Motte2003}
}
\label{pointings}      % is used to refer this table in the text
\begin{tabular}{c c c}        % centered columns (4 columns)
\hline\hline                 % inserts double horizontal lines
Offsets & Column Density  \\     % table heading
[(arcsec, arcsec)] &  [cm$^{-2}$]  \\
\hline                        % inserts single horizontal line
   (0,20) & $1.3 \times 10^{24}$ \\   % inserting body of the tabl
   (20,30) & $1.4 \times 10^{23}$ \\
   (0,0) & $1.5 \times 10^{14}$ \\
   (-30,-20) & $3.7 \times 10^{23}$ \\
\hline                                    %inserts single line
\end{tabular}
\end{table*}

